RG Flows and Thermofield-Double States in Holography

In this article, we consider a Renormalization Group flow of the Thermofield-Double state in a UV-complete description of Holography, by introducing a relevant deformation to the ${\cal N}=4$ super Yang-Mills theory at strong coupling. This RG-flow is known to have a non-trivial, interacting ${\cal N}=1$ fixed point at the IR. Geometrically, an RG-flow of the TFD-state naturally continues radially and inside the black hole event horizon and yields a Kasner-structure near singularity, as has been observed in recent works. We show that for a generic value of the deformation, the putative IR fixed point remains inside the black hole. By fine-tuning this deformation, the "fixed point" can be brought arbitrarily close to the event horizon, while always remaining inside. Physically, this distinguishes between the vanishing temperature limit of the RG-flows with the one at exactly zero temperature. We further discuss its general implications in the context of Holography. We also discuss how correlations between the two-copies of the TFD-state depend on this explicit RG-flow.

==> RG FLOW FINAL/bibliography1.tex <==

@article{Maldacena:2001kr,
    author = "Maldacena, Juan Martin",
    title = "{Eternal black holes in anti-de Sitter}",
    eprint = "hep-th/0106112",
    archivePrefix = "arXiv",
    reportNumber = "NSF-ITP-01-59",
    doi = "10.1088/1126-6708/2003/04/021",
    journal = "JHEP",
    volume = "04",
    pages = "021",
    year = "2003"

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


@article{Frenkel:2020ysx,
    author = "Frenkel, Alexander and Hartnoll, Sean A. and Kruthoff, Jorrit and Shi, Zhengyan D.",
    title = "{Holographic flows from CFT to the Kasner universe}",
    eprint = "2004.01192",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.1007/JHEP08(2020)003",
    journal = "JHEP",
    volume = "08",
    pages = "003",
    year = "2020"

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 

@article{Kasner:1921zz,
    author = "Kasner, Edward",
    title = "{Geometrical theorems on Einstein's cosmological equations}",
    doi = "10.2307/2370192",
    journal = "Am. J. Math.",
    volume = "43",
    pages = "217--221",
    year = "1921"

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


@article{Kiritsis:2016kog,
    author = "Kiritsis, Elias and Nitti, Francesco and Silva Pimenta, Leandro",
    title = "{Exotic RG Flows from Holography}",
    eprint = "1611.05493",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.1002/prop.201600120",
    journal = "Fortsch. Phys.",
    volume = "65",
    number = "2",
    pages = "1600120",
    year = "2017"

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


@article{Maldacena:1997re,
    author = "Maldacena, Juan Martin",
    title = "{The Large N limit of superconformal field theories and supergravity}",
    eprint = "hep-th/9711200",
    archivePrefix = "arXiv",
    reportNumber = "HUTP-97-A097, HUTP-98-A097",
    doi = "10.1023/A:1026654312961",
    journal = "Adv. Theor. Math. Phys.",
    volume = "2",
    pages = "231--252",
    year = "1998"

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

@article{frenkel2020holographic,
  title={Holographic flows from CFT to the Kasner universe},
  author={Frenkel, Alexander and Hartnoll, Sean A and Kruthoff, Jorrit and Shi, Zhengyan D},
  journal={Journal of High Energy Physics},
  volume={2020},
  number={8},
  pages={1--19},
  year={2020},
  publisher={Springer}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

@article{Freedman:1999gp,
    author = "Freedman, D. Z. and Gubser, S. S. and Pilch, K. and Warner, N. P.",
    title = "{Renormalization group flows from holography supersymmetry and a c theorem}",
    eprint = "hep-th/9904017",
    archivePrefix = "arXiv",
    reportNumber = "CERN-TH-99-86, HUTP-99-A015, USC-99-1, MIT-CTP-2846",
    doi = "10.4310/ATMP.1999.v3.n2.a7",
    journal = "Adv. Theor. Math. Phys.",
    volume = "3",
    pages = "363--417",
    year = "1999"

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

@article{Siopsis:2010pi,
    author = "Siopsis, George and Therrien, Jason and Musiri, Suphot",
    title = "{Holographic superconductors near the Breitenlohner-Freedman bound}",
    eprint = "1011.2938",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    reportNumber = "UTHET-10-1001",
    doi = "10.1088/0264-9381/29/8/085007",
    journal = "Class. Quant. Grav.",
    volume = "29",
    pages = "085007",
    year = "2012"


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

@article{Faulkner:2010jy,
    author = "Faulkner, Thomas and Liu, Hong and Rangamani, Mukund",
    title = "{Integrating out geometry: Holographic Wilsonian RG and the membrane paradigm}",
    eprint = "1010.4036",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    reportNumber = "MIT-CTP-4185, DCPT-10-47",
    doi = "10.1007/JHEP08(2011)051",
    journal = "JHEP",
    volume = "08",
    pages = "051",
    year = "2011"
    
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

@article{Leutheusser:2021qhd,
    author = "Leutheusser, Samuel and Liu, Hong",
    title = "{Causal connectability between quantum systems and the black hole interior in holographic duality}",
    eprint = "2110.05497",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    reportNumber = "MIT-CTP/5335",
    month = "10",
    year = "2021"
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

@article{Anand:2017yij,
    author = "Anand, Nikhil and Genest, Vincent X. and Katz, Emanuel and Khandker, Zuhair U. and Walters, Matthew T.",
    title = "{RG flow from $\phi^4$ theory to the 2D Ising model}",
    eprint = "1704.04500",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.1007/JHEP08(2017)056",
    journal = "JHEP",
    volume = "08",
    pages = "056",
    year = "2017"
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

@article{Israel:1976ur,
    author = "Israel, W.",
    title = "{Thermo field dynamics of black holes}",
    doi = "10.1016/0375-9601(76)90178-X",
    journal = "Phys. Lett. A",
    volume = "57",
    pages = "107--110",
    year = "1976"
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

@article{Cotler:2016fpe,
    author = "Cotler, Jordan S. and Gur-Ari, Guy and Hanada, Masanori and Polchinski, Joseph and Saad, Phil and Shenker, Stephen H. and Stanford, Douglas and Streicher, Alexandre and Tezuka, Masaki",
    title = "{Black Holes and Random Matrices}",
    eprint = "1611.04650",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    reportNumber = "SU-ITP-16-19, SU-ITP-16/19, YITP-16-124",
    doi = "10.1007/JHEP05(2017)118",
    journal = "JHEP",
    volume = "05",
    pages = "118",
    year = "2017",
    note = "[Erratum: JHEP 09, 002 (2018)]"
}




@article{Faulkner:2010jy,
    author = "Faulkner, Thomas and Liu, Hong and Rangamani, Mukund",
    title = "{Integrating out geometry: Holographic Wilsonian RG and the membrane paradigm}",
    eprint = "1010.4036",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    reportNumber = "MIT-CTP-4185, DCPT-10-47",
    doi = "10.1007/JHEP08(2011)051",
    journal = "JHEP",
    volume = "08",
    pages = "051",
    year = "2011"
}




@article{Gao:2018yzk,
    author = "Gao, Ping and Liu, Hong",
    title = "{Regenesis and quantum traversable wormholes}",
    eprint = "1810.01444",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.1007/JHEP10(2019)048",
    journal = "JHEP",
    volume = "10",
    pages = "048",
    year = "2019"
}



@article{Gao:2016bin,
    author = "Gao, Ping and Jafferis, Daniel Louis and Wall, Aron C.",
    title = "{Traversable Wormholes via a Double Trace Deformation}",
    eprint = "1608.05687",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.1007/JHEP12(2017)151",
    journal = "JHEP",
    volume = "12",
    pages = "151",
    year = "2017"
}



@article{Kundu:2021nwp,
    author = "Kundu, Arnab",
    title = "{Wormholes \& Holography: An Introduction}",
    eprint = "2110.14958",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    month = "10",
    year = "2021"
}



@article{Hartnoll:2020rwq,
    author = "Hartnoll, Sean A. and Horowitz, Gary T. and Kruthoff, Jorrit and Santos, Jorge E.",
    title = "{Gravitational duals to the grand canonical ensemble abhor Cauchy horizons}",
    eprint = "2006.10056",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.1007/JHEP10(2020)102",
    journal = "JHEP",
    volume = "10",
    pages = "102",
    year = "2020"
}


@article{Hartnoll:2020fhc,
    author = "Hartnoll, Sean A. and Horowitz, Gary T. and Kruthoff, Jorrit and Santos, Jorge E.",
    title = "{Diving into a holographic superconductor}",
    eprint = "2008.12786",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.21468/SciPostPhys.10.1.009",
    journal = "SciPost Phys.",
    volume = "10",
    number = "1",
    pages = "009",
    year = "2021"
}


@article{Caceres:2021fuw,
    author = "Caceres, Elena and Kundu, Arnab and Patra, Ayan K. and Shashi, Sanjit",
    title = "{Page Curves and Bath Deformations}",
    eprint = "2107.00022",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    month = "6",
    year = "2021"
}


@article{Bhattacharya:2021nqj,
    author = "Bhattacharya, Aranya and Bhattacharyya, Arpan and Nandy, Pratik and Patra, Ayan K.",
    title = "{Bath deformations, islands and holographic complexity}",
    eprint = "2112.06967",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    month = "12",
    year = "2021"
}


@article{2006,
   title={Entanglement and the foundations of statistical mechanics},
   volume={2},
   ISSN={1745-2481},
   url={http://dx.doi.org/10.1038/nphys444},
   DOI={10.1038/nphys444},
   number={11},
   journal={Nature Physics},
   publisher={Springer Science and Business Media LLC},
   author={Popescu, Sandu and Short, Anthony J. and Winter, Andreas},
   year={2006},
   month={Oct},
   pages={754–758}
}



@article{Casini:2006es,
    author = "Casini, H. and Huerta, M.",
    editor = "Sola, Joan",
    title = "{A c-theorem for the entanglement entropy}",
    eprint = "cond-mat/0610375",
    archivePrefix = "arXiv",
    doi = "10.1088/1751-8113/40/25/S57",
    journal = "J. Phys. A",
    volume = "40",
    pages = "7031--7036",
    year = "2007"
}



@article{Casini:2012ei,
    author = "Casini, H. and Huerta, Marina",
    title = "{On the RG running of the entanglement entropy of a circle}",
    eprint = "1202.5650",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.1103/PhysRevD.85.125016",
    journal = "Phys. Rev. D",
    volume = "85",
    pages = "125016",
    year = "2012"
}


@article{Casini:2016fgb,
    author = "Casini, Horacio and Salazar Landea, Ignacio and Torroba, Gonzalo",
    title = "{The g-theorem and quantum information theory}",
    eprint = "1607.00390",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.1007/JHEP10(2016)140",
    journal = "JHEP",
    volume = "10",
    pages = "140",
    year = "2016"
}



@article{Albash:2011nq,
    author = "Albash, Tameem and Johnson, Clifford V.",
    title = "{Holographic Entanglement Entropy and Renormalization Group Flow}",
    eprint = "1110.1074",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.1007/JHEP02(2012)095",
    journal = "JHEP",
    volume = "02",
    pages = "095",
    year = "2012"
}



@article{Kundu:2020nir,
    author = "Kundu, Arnab",
    title = "{Fast Scrambling under an RG-flow}",
    eprint = "2006.11037",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    month = "6",
    year = "2020"
}


@article{Ryu:2006bv,
    author = "Ryu, Shinsei and Takayanagi, Tadashi",
    title = "{Holographic derivation of entanglement entropy from AdS/CFT}",
    eprint = "hep-th/0603001",
    archivePrefix = "arXiv",
    reportNumber = "NSF-KITP-06-11",
    doi = "10.1103/PhysRevLett.96.181602",
    journal = "Phys. Rev. Lett.",
    volume = "96",
    pages = "181602",
    year = "2006"
}



@article{Hubeny:2007xt,
    author = "Hubeny, Veronika E. and Rangamani, Mukund and Takayanagi, Tadashi",
    title = "{A Covariant holographic entanglement entropy proposal}",
    eprint = "0705.0016",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    reportNumber = "DCPT-07-13, KUNS-2069",
    doi = "10.1088/1126-6708/2007/07/062",
    journal = "JHEP",
    volume = "07",
    pages = "062",
    year = "2007"
}


@article{Hartman:2013qma,
    author = "Hartman, Thomas and Maldacena, Juan",
    title = "{Time Evolution of Entanglement Entropy from Black Hole Interiors}",
    eprint = "1303.1080",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.1007/JHEP05(2013)014",
    journal = "JHEP",
    volume = "05",
    pages = "014",
    year = "2013"
}


@article{Leigh:1995ep,
    author = "Leigh, Robert G. and Strassler, Matthew J.",
    title = "{Exactly marginal operators and duality in four-dimensional N=1 supersymmetric gauge theory}",
    eprint = "hep-th/9503121",
    archivePrefix = "arXiv",
    reportNumber = "RU-95-2",
    doi = "10.1016/0550-3213(95)00261-P",
    journal = "Nucl. Phys. B",
    volume = "447",
    pages = "95--136",
    year = "1995"
}



@article{CKPS:2022,
    author = "Caceres, Elena and Kundu, Arnab and Patra, Ayan K. and Shashi, Sanjit",
    title = "{To appear}",
%    eprint = "hep-th/9503121",
%    archivePrefix = "arXiv",
%    reportNumber = "RU-95-2",
%    doi = "10.1016/0550-3213(95)00261-P",
%    journal = "Nucl. Phys. B",
%    volume = "447",
%    pages = "95--136",
%    year = "1995"
}



@article{Maldacena:2017axo,
    author = "Maldacena, Juan and Stanford, Douglas and Yang, Zhenbin",
    title = "{Diving into traversable wormholes}",
    eprint = "1704.05333",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.1002/prop.201700034",
    journal = "Fortsch. Phys.",
    volume = "65",
    number = "5",
    pages = "1700034",
    year = "2017"
}


@article{2021,
   title={Entanglement Renormalization of Thermofield Double States},
   volume={127},
   ISSN={1079-7114},
   url={http://dx.doi.org/10.1103/PhysRevLett.127.080602},
   DOI={10.1103/physrevlett.127.080602},
   number={8},
   journal={Physical Review Letters},
   publisher={American Physical Society (APS)},
   author={Lin, Cheng-Ju and Li, Zhi and Hsieh, Timothy H.},
   year={2021},
   month={Aug}
}







==> bibliography1.tex <==

@article{Maldacena:2001kr,
    author = "Maldacena, Juan Martin",
    title = "{Eternal black holes in anti-de Sitter}",
    eprint = "hep-th/0106112",
    archivePrefix = "arXiv",
    reportNumber = "NSF-ITP-01-59",
    doi = "10.1088/1126-6708/2003/04/021",
    journal = "JHEP",
    volume = "04",
    pages = "021",
    year = "2003"

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


@article{Frenkel:2020ysx,
    author = "Frenkel, Alexander and Hartnoll, Sean A. and Kruthoff, Jorrit and Shi, Zhengyan D.",
    title = "{Holographic flows from CFT to the Kasner universe}",
    eprint = "2004.01192",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.1007/JHEP08(2020)003",
    journal = "JHEP",
    volume = "08",
    pages = "003",
    year = "2020"

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 

@article{Kasner:1921zz,
    author = "Kasner, Edward",
    title = "{Geometrical theorems on Einstein's cosmological equations}",
    doi = "10.2307/2370192",
    journal = "Am. J. Math.",
    volume = "43",
    pages = "217--221",
    year = "1921"

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


@article{Kiritsis:2016kog,
    author = "Kiritsis, Elias and Nitti, Francesco and Silva Pimenta, Leandro",
    title = "{Exotic RG Flows from Holography}",
    eprint = "1611.05493",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.1002/prop.201600120",
    journal = "Fortsch. Phys.",
    volume = "65",
    number = "2",
    pages = "1600120",
    year = "2017"

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


@article{Maldacena:1997re,
    author = "Maldacena, Juan Martin",
    title = "{The Large N limit of superconformal field theories and supergravity}",
    eprint = "hep-th/9711200",
    archivePrefix = "arXiv",
    reportNumber = "HUTP-97-A097, HUTP-98-A097",
    doi = "10.1023/A:1026654312961",
    journal = "Adv. Theor. Math. Phys.",
    volume = "2",
    pages = "231--252",
    year = "1998"

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

@article{frenkel2020holographic,
  title={Holographic flows from CFT to the Kasner universe},
  author={Frenkel, Alexander and Hartnoll, Sean A and Kruthoff, Jorrit and Shi, Zhengyan D},
  journal={Journal of High Energy Physics},
  volume={2020},
  number={8},
  pages={1--19},
  year={2020},
  publisher={Springer}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

@article{Freedman:1999gp,
    author = "Freedman, D. Z. and Gubser, S. S. and Pilch, K. and Warner, N. P.",
    title = "{Renormalization group flows from holography supersymmetry and a c theorem}",
    eprint = "hep-th/9904017",
    archivePrefix = "arXiv",
    reportNumber = "CERN-TH-99-86, HUTP-99-A015, USC-99-1, MIT-CTP-2846",
    doi = "10.4310/ATMP.1999.v3.n2.a7",
    journal = "Adv. Theor. Math. Phys.",
    volume = "3",
    pages = "363--417",
    year = "1999"

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

@article{Siopsis:2010pi,
    author = "Siopsis, George and Therrien, Jason and Musiri, Suphot",
    title = "{Holographic superconductors near the Breitenlohner-Freedman bound}",
    eprint = "1011.2938",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    reportNumber = "UTHET-10-1001",
    doi = "10.1088/0264-9381/29/8/085007",
    journal = "Class. Quant. Grav.",
    volume = "29",
    pages = "085007",
    year = "2012"


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

@article{Faulkner:2010jy,
    author = "Faulkner, Thomas and Liu, Hong and Rangamani, Mukund",
    title = "{Integrating out geometry: Holographic Wilsonian RG and the membrane paradigm}",
    eprint = "1010.4036",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    reportNumber = "MIT-CTP-4185, DCPT-10-47",
    doi = "10.1007/JHEP08(2011)051",
    journal = "JHEP",
    volume = "08",
    pages = "051",
    year = "2011"
    
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

@article{Leutheusser:2021qhd,
    author = "Leutheusser, Samuel and Liu, Hong",
    title = "{Causal connectability between quantum systems and the black hole interior in holographic duality}",
    eprint = "2110.05497",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    reportNumber = "MIT-CTP/5335",
    month = "10",
    year = "2021"
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

@article{Anand:2017yij,
    author = "Anand, Nikhil and Genest, Vincent X. and Katz, Emanuel and Khandker, Zuhair U. and Walters, Matthew T.",
    title = "{RG flow from $\phi^4$ theory to the 2D Ising model}",
    eprint = "1704.04500",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.1007/JHEP08(2017)056",
    journal = "JHEP",
    volume = "08",
    pages = "056",
    year = "2017"
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

@article{Israel:1976ur,
    author = "Israel, W.",
    title = "{Thermo field dynamics of black holes}",
    doi = "10.1016/0375-9601(76)90178-X",
    journal = "Phys. Lett. A",
    volume = "57",
    pages = "107--110",
    year = "1976"
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

@article{Cotler:2016fpe,
    author = "Cotler, Jordan S. and Gur-Ari, Guy and Hanada, Masanori and Polchinski, Joseph and Saad, Phil and Shenker, Stephen H. and Stanford, Douglas and Streicher, Alexandre and Tezuka, Masaki",
    title = "{Black Holes and Random Matrices}",
    eprint = "1611.04650",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    reportNumber = "SU-ITP-16-19, SU-ITP-16/19, YITP-16-124",
    doi = "10.1007/JHEP05(2017)118",
    journal = "JHEP",
    volume = "05",
    pages = "118",
    year = "2017",
    note = "[Erratum: JHEP 09, 002 (2018)]"
}




@article{Faulkner:2010jy,
    author = "Faulkner, Thomas and Liu, Hong and Rangamani, Mukund",
    title = "{Integrating out geometry: Holographic Wilsonian RG and the membrane paradigm}",
    eprint = "1010.4036",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    reportNumber = "MIT-CTP-4185, DCPT-10-47",
    doi = "10.1007/JHEP08(2011)051",
    journal = "JHEP",
    volume = "08",
    pages = "051",
    year = "2011"
}




@article{Gao:2018yzk,
    author = "Gao, Ping and Liu, Hong",
    title = "{Regenesis and quantum traversable wormholes}",
    eprint = "1810.01444",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.1007/JHEP10(2019)048",
    journal = "JHEP",
    volume = "10",
    pages = "048",
    year = "2019"
}



@article{Gao:2016bin,
    author = "Gao, Ping and Jafferis, Daniel Louis and Wall, Aron C.",
    title = "{Traversable Wormholes via a Double Trace Deformation}",
    eprint = "1608.05687",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.1007/JHEP12(2017)151",
    journal = "JHEP",
    volume = "12",
    pages = "151",
    year = "2017"
}



@article{Kundu:2021nwp,
    author = "Kundu, Arnab",
    title = "{Wormholes \& Holography: An Introduction}",
    eprint = "2110.14958",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    month = "10",
    year = "2021"
}



@article{Hartnoll:2020rwq,
    author = "Hartnoll, Sean A. and Horowitz, Gary T. and Kruthoff, Jorrit and Santos, Jorge E.",
    title = "{Gravitational duals to the grand canonical ensemble abhor Cauchy horizons}",
    eprint = "2006.10056",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.1007/JHEP10(2020)102",
    journal = "JHEP",
    volume = "10",
    pages = "102",
    year = "2020"
}


@article{Hartnoll:2020fhc,
    author = "Hartnoll, Sean A. and Horowitz, Gary T. and Kruthoff, Jorrit and Santos, Jorge E.",
    title = "{Diving into a holographic superconductor}",
    eprint = "2008.12786",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.21468/SciPostPhys.10.1.009",
    journal = "SciPost Phys.",
    volume = "10",
    number = "1",
    pages = "009",
    year = "2021"
}


@article{Caceres:2021fuw,
    author = "Caceres, Elena and Kundu, Arnab and Patra, Ayan K. and Shashi, Sanjit",
    title = "{Page Curves and Bath Deformations}",
    eprint = "2107.00022",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    month = "6",
    year = "2021"
}


@article{Bhattacharya:2021nqj,
    author = "Bhattacharya, Aranya and Bhattacharyya, Arpan and Nandy, Pratik and Patra, Ayan K.",
    title = "{Bath deformations, islands and holographic complexity}",
    eprint = "2112.06967",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    month = "12",
    year = "2021"
}


@article{2006,
   title={Entanglement and the foundations of statistical mechanics},
   volume={2},
   ISSN={1745-2481},
   url={http://dx.doi.org/10.1038/nphys444},
   DOI={10.1038/nphys444},
   number={11},
   journal={Nature Physics},
   publisher={Springer Science and Business Media LLC},
   author={Popescu, Sandu and Short, Anthony J. and Winter, Andreas},
   year={2006},
   month={Oct},
   pages={754–758}
}



@article{Casini:2006es,
    author = "Casini, H. and Huerta, M.",
    editor = "Sola, Joan",
    title = "{A c-theorem for the entanglement entropy}",
    eprint = "cond-mat/0610375",
    archivePrefix = "arXiv",
    doi = "10.1088/1751-8113/40/25/S57",
    journal = "J. Phys. A",
    volume = "40",
    pages = "7031--7036",
    year = "2007"
}



@article{Casini:2012ei,
    author = "Casini, H. and Huerta, Marina",
    title = "{On the RG running of the entanglement entropy of a circle}",
    eprint = "1202.5650",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.1103/PhysRevD.85.125016",
    journal = "Phys. Rev. D",
    volume = "85",
    pages = "125016",
    year = "2012"
}


@article{Casini:2016fgb,
    author = "Casini, Horacio and Salazar Landea, Ignacio and Torroba, Gonzalo",
    title = "{The g-theorem and quantum information theory}",
    eprint = "1607.00390",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.1007/JHEP10(2016)140",
    journal = "JHEP",
    volume = "10",
    pages = "140",
    year = "2016"
}



@article{Albash:2011nq,
    author = "Albash, Tameem and Johnson, Clifford V.",
    title = "{Holographic Entanglement Entropy and Renormalization Group Flow}",
    eprint = "1110.1074",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.1007/JHEP02(2012)095",
    journal = "JHEP",
    volume = "02",
    pages = "095",
    year = "2012"
}



@article{Kundu:2020nir,
    author = "Kundu, Arnab",
    title = "{Fast Scrambling under an RG-flow}",
    eprint = "2006.11037",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    month = "6",
    year = "2020"
}


@article{Ryu:2006bv,
    author = "Ryu, Shinsei and Takayanagi, Tadashi",
    title = "{Holographic derivation of entanglement entropy from AdS/CFT}",
    eprint = "hep-th/0603001",
    archivePrefix = "arXiv",
    reportNumber = "NSF-KITP-06-11",
    doi = "10.1103/PhysRevLett.96.181602",
    journal = "Phys. Rev. Lett.",
    volume = "96",
    pages = "181602",
    year = "2006"
}



@article{Hubeny:2007xt,
    author = "Hubeny, Veronika E. and Rangamani, Mukund and Takayanagi, Tadashi",
    title = "{A Covariant holographic entanglement entropy proposal}",
    eprint = "0705.0016",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    reportNumber = "DCPT-07-13, KUNS-2069",
    doi = "10.1088/1126-6708/2007/07/062",
    journal = "JHEP",
    volume = "07",
    pages = "062",
    year = "2007"
}


@article{Hartman:2013qma,
    author = "Hartman, Thomas and Maldacena, Juan",
    title = "{Time Evolution of Entanglement Entropy from Black Hole Interiors}",
    eprint = "1303.1080",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.1007/JHEP05(2013)014",
    journal = "JHEP",
    volume = "05",
    pages = "014",
    year = "2013"
}


@article{Leigh:1995ep,
    author = "Leigh, Robert G. and Strassler, Matthew J.",
    title = "{Exactly marginal operators and duality in four-dimensional N=1 supersymmetric gauge theory}",
    eprint = "hep-th/9503121",
    archivePrefix = "arXiv",
    reportNumber = "RU-95-2",
    doi = "10.1016/0550-3213(95)00261-P",
    journal = "Nucl. Phys. B",
    volume = "447",
    pages = "95--136",
    year = "1995"
}



@article{CKPS:2022,
    author = "Caceres, Elena and Kundu, Arnab and Patra, Ayan K. and Shashi, Sanjit",
    title = "{To appear}",
%    eprint = "hep-th/9503121",
%    archivePrefix = "arXiv",
%    reportNumber = "RU-95-2",
%    doi = "10.1016/0550-3213(95)00261-P",
%    journal = "Nucl. Phys. B",
%    volume = "447",
%    pages = "95--136",
%    year = "1995"
}



@article{Maldacena:2017axo,
    author = "Maldacena, Juan and Stanford, Douglas and Yang, Zhenbin",
    title = "{Diving into traversable wormholes}",
    eprint = "1704.05333",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.1002/prop.201700034",
    journal = "Fortsch. Phys.",
    volume = "65",
    number = "5",
    pages = "1700034",
    year = "2017"
}


@article{2021,
   title={Entanglement Renormalization of Thermofield Double States},
   volume={127},
   ISSN={1079-7114},
   url={http://dx.doi.org/10.1103/PhysRevLett.127.080602},
   DOI={10.1103/physrevlett.127.080602},
   number={8},
   journal={Physical Review Letters},
   publisher={American Physical Society (APS)},
   author={Lin, Cheng-Ju and Li, Zhi and Hsieh, Timothy H.},
   year={2021},
   month={Aug}
}






